Hot super-Earths stripped by their host stars

Simulations predict that hot super-Earth sized exoplanets can have their envelopes stripped by photo-evaporation, which would present itself as a lack of these exoplanets. However, this absence in the exoplanet population has escaped a firm detection. Here we demonstrate, using asteroseismology on a sample of exoplanets and exoplanet candidates observed during the Kepler mission that, while there is an abundance of super-Earth sized exoplanets with low incident fluxes, none are found with high incident fluxes. We do not find any exoplanets with radii between 2.2 and 3.8 Earth radii with incident flux above 650 times the incident flux on Earth. This gap in the population of exoplanets is explained by evaporation of volatile elements and thus supports the predictions. The confirmation of a hot-super-Earth desert caused by evaporation will add an important constraint on simulations of planetary systems, since they must be able to reproduce the dearth of close-in super-Earths.

==> journal_abreviations.tex <==
% From aastex.cls (from line 1728) - journal abreviations:
\makeatletter
\let\jnl@style=\rmfamily
\def\ref@jnl#1{{\jnl@style#1}}%
\newcommand\aj{\ref@jnl{AJ}}%
          % Astronomical Journal
\newcommand\actaa{\ref@jnl{Acta Astron.}}%
  % Acta Astronomica
\newcommand\araa{\ref@jnl{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\ref@jnl{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\ref@jnl{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\ref@jnl{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\ref@jnl{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\ref@jnl{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\ref@jnl{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\ref@jnl{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\ref@jnl{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\ref@jnl{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\ref@jnl{BAAS}}%
          % Bulletin of the AAS
\newcommand\caa{\ref@jnl{Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\ref@jnl{Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{\ref@jnl{Icarus}}%
  % Icarus
\newcommand\jcap{\ref@jnl{J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{\ref@jnl{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\ref@jnl{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\ref@jnl{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\na{\ref@jnl{New A}}%
  % New Astronomy
\newcommand\nar{\ref@jnl{New A Rev.}}%
  % New Astronomy Review
\newcommand\pra{\ref@jnl{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\ref@jnl{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\ref@jnl{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\ref@jnl{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\ref@jnl{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\ref@jnl{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasa{\ref@jnl{PASA}}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{\ref@jnl{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\ref@jnl{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\ref@jnl{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{\ref@jnl{Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{\ref@jnl{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\ref@jnl{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\ref@jnl{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\ref@jnl{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\ref@jnl{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\ref@jnl{Nature}}%
          % Nature
\newcommand\iaucirc{\ref@jnl{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\ref@jnl{Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
\newcommand\apspr{\ref@jnl{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\ref@jnl{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\ref@jnl{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\ref@jnl{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\ref@jnl{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\ref@jnl{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\ref@jnl{J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
\newcommand\jqsrt{\ref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\ref@jnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\ref@jnl{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\ref@jnl{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\ref@jnl{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\ref@jnl{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\ref@jnl{Proc.~SPIE}}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

\makeatother
